Machine Learned Interatomic Potential for Dispersion Strengthened Plasma Facing Components

Tungsten (W) is a material of choice for the divertor material due to its high melting temperature, thermal conductivity, and sputtering threshold. However, W has a very high brittle-to-ductile transition temperature and at fusion reactor temperatures ($\geq$1000K) may undergo recrystallization and grain growth. Dispersion-strengthening W with zirconium carbide (ZrC) can improve ductility and limit grain growth, but much of the effects of the dispersoids on microstructural evolution and thermomechanical properties at high temperature are still unknown. We present a machine learned Spectral Neighbor Analysis Potential (SNAP) for W-ZrC that can now be used to study these materials. In order to construct a potential suitable for large-scale atomistic simulations at fusion reactor temperatures, it is necessary to train on ab initio data generated for a diverse set of structures, chemical environments, and temperatures. Further accuracy and stability tests of the potential were achieved using objective functions for both material properties and high temperature stability. Validation of lattice parameters, surface energies, bulk moduli, and thermal expansion is confirmed on the optimized potential. Tensile tests of W/ZrC bicrystals show that while the W(110)-ZrC(111) C-terminated bicrystal has the highest ultimate tensile strength (UTS) at room temperature, observed strength decreases with increasing temperature. At 2500K, the terminating C layer diffuses into the W, resulting in a weaker W-Zr interface. Meanwhile, the W(110)-ZrC(111) Zr-terminated bicrystal has the highest UTS at 2500K.

==> Tables_WBe_PRB.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcclllcclllccll}
Description&$N_{E}$&$N_{F}$&$\sigma_{E}$&$\sigma_{F}$&Description&$N_{E}$&$N_{F}$&$\sigma_{E}$&$\sigma_{F}$&Description&$N_{E}$&$N_{F}$&$\sigma_{E}$&$\sigma_{F}$\\
\hline
\hline
W:&&&&&Be:&&&&&W-Be:\\
Elastic Deform & 2000 & 6000 & $5\cdot10^{0}$ & $6\cdot10^{4}$ & Elastic Deform & 4594 & 43260 & $1\cdot10^{5}$ & $\bf{1\cdot10^{7}}$ & Elastic Deform$^{\dagger}$ & 3946 & 68040 & $\bf{3\cdot10^{5}}$ & $2\cdot10^{3}$\\
Equation of State & 125 & 3468 & $1\cdot10^{-1}$ & $6\cdot10^{4}$ & Equation of State & 502 & 5418 & $6\cdot10^{4}$ & $3\cdot10^{6}$ & Equation of State$^{\dagger}$ & 1113 & 39627 & $2\cdot10^{5}$ &$4\cdot10^{4}$ \\ 
DFT-MD & 60 & 23040 & $3\cdot10^{0}$ & $1\cdot10^{4}$ & DFT-MD & 909 & 130896 & $\bf{2\cdot10^{5}}$ & $2\cdot10^{6}$ & DFT-MD$^{\dagger}$ & 3360 & 497124 & $7\cdot10^{4}$ & $6\cdot10^{2}$ \\
Surfaces & 180 & 334818 & $\bf{1\cdot10^{5}}$ & $3\cdot10^{5}$ & Surfaces & 90 & 17280 & $1\cdot10^{3}$ & $4\cdot10^{5}$& Surface Adhesion & 381 & 112527 & $2\cdot10^{4}$ & $\bf{9\cdot10^{4}}$ \\ 
Self-Interstitials &15 &5805 & $5\cdot10^{-2}$ & $8\cdot10^{2}$ & Self-Interstitials & 179 & 137931 & $3\cdot10^{2}$ & $4\cdot10^{5}$  & \multicolumn{5}{l}{$\dagger$ multiple crystal phases included in this group:}\\
Liquids & 27 & 3120	&$4\cdot10^{-3}$ & $3\cdot10^{2}$ & Liquids & 75 & 57600 & $7\cdot10^{1}$ & $7\cdot10^{5}$ \\
Dislocations & 98 & 39690 & $3\cdot10^{0}$ & $9\cdot10^{4}$ & Stacking Faults & 6 & 864 & $3\cdot10^{0}$ & $2\cdot10^{6}$ \\
Monovacancy & 420 	& 183054 & $2\cdot10^{3}$ & $1\cdot10^{5}$ &&&&&& \multirow{3}{*}[0.3875in]{ \begin{minipage}{1mm} \includegraphics[]{WBe_Phases.png} \end{minipage}}\\
Divacancy	 & 39	& 6084 & $1\cdot10^{0}$ & $1\cdot10^{3}$ \\
$\Gamma$-Surface & 6183 & 328338 & $1\cdot10^{0}$ & $1\cdot10^{6}$  \\
$\Gamma$-Surf.+Vacancy & 750 & 105750 & $4\cdot10^{-1}$ & $\bf{3\cdot10^{6}}$ \\
\hline
Total&9897&1039167&&&&6355&393249&&&&8800&717318&&\\
\end{tabular}}
\caption{Training data used in the full W-Be SNAP fit, broken down by element type and group within each element. 
%A group is defined by similarity of the DFT calculations in terms of the atomic configuration used as input. 
%Listed from top to bottom are groups that represent more equilibrium material properties onto defect/low symmetry configurations. 
Each of the groups in the W-Be category contain configurations for multiple inter-metallic compounds, some of which are displayed in the inset. For each group the number of energy ($N_E$) and force ($N_F$) training points are given as well as the optimal training weight ($\sigma_E, \sigma_F$) selected for the full W-Be SNAP potential.}
\label{table:alltrain}
\end{table*}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcclcclcc}
Description&$\Delta E (eV/atom)$&$\Delta F (eV/\AA)$&Description&$\Delta E (eV/atom)$&$\Delta F (eV/\AA)$&Description&$\Delta E (eV/atom)$&$\Delta F (eV/\AA)$\\
\hline
\hline
W:&&&Be:&&&W-Be:\\
Elastic Deform & $5.3\cdot10^{-2}$ & $0.0\cdot10^{0}$ & Elastic Deform & $7.6\cdot10^{-2}$ & $2.3\cdot10^{-3}$ & Elastic Deform$^{\dagger}$ & $9.2\cdot10^{-2}$ & $\uline{1.7\cdot10^{-1}}$ \\
Equation of State & $1.4\cdot10^{-1}$ & $\uline{4.0\cdot10^{-5}}$ & Equation of State & $9.8\cdot10^{-2}$ & $\uline{8.8\cdot10^{-4}}$ & Equation of State$^{\dagger}$ & $\bf{1.1\cdot10^{0}}$ & $\bf{6.3\cdot10^{-1}}$ \\ 
DFT-MD & $5.3\cdot10^{-2}$ & $6.0\cdot10^{-2}$ & DFT-MD & $3.6\cdot10^{-2}$ & $8.2\cdot10^{-2}$ & DFT-MD$^{\dagger}$ & $\uline{7.9\cdot10^{-2}}$ & $5.7\cdot10^{-1}$ \\
Surfaces & $3.4\cdot10^{-2}$ & $2.8\cdot10^{-1}$ & Surfaces & $\uline{1.8\cdot10^{-2}}$ & $5.0\cdot10^{-2}$ &Surface Adhesion & $8.6\cdot10^{-2}$ & $4.7\cdot10^{-1}$ \\ 
Self-Interstitials &$4.6\cdot10^{-2}$ & $9.5\cdot10^{-2}$ & Self-Interstitials & $\bf{1.3\cdot10^{0}}$ & $8.2\cdot10^{-2}$ & \multicolumn{3}{l}{$\dagger$ Multiple crystal phases included in this group}\\
Liquids & $\bf{2.9\cdot10^{-1}}$ & $\bf{4.8\cdot10^{-1}}$ & Liquids & $6.5\cdot10^{-2}$ & $\bf{2.6\cdot10^{-1}}$  \\
Dislocations & $5.0\cdot10^{-2}$ & $7.8\cdot10^{-2}$ & Stacking Faults & $2.0\cdot10^{-2}$ & $2.0\cdot10^{-3}$ \\
Monovacancy & $4.2\cdot10^{-2}$ & $9.8\cdot10^{-2}$ &&&&&& \\
Divacancy	 & $\uline{2.9\cdot10^{-2}}$ & $8.7\cdot10^{-2}$ \\
$\Gamma$-Surface & $4.6\cdot10^{-2}$ & $2.5\cdot10^{-1}$ \\
$\Gamma$-Surf.+Vacancy & $4.3\cdot10^{-2}$ & $1.7\cdot10^{-1}$ \\
\hline
\end{tabular}}
\caption{Regression errors for training data used in the full W-Be SNAP fit, broken down by element type and group within each element. Within each elemental set of training data values are bolded and underlined for the highest and lowest error values, respectively. Force errors for the tungsten elastic deformations are zero due to the fact a single atom unit cell was used in these DFT calculations and all forces are identically zero.}
\label{table:errtrain}
\end{table*}

==> WNbib <==
% Initial references taken from W-Be potential paper and W-Be-He paper


@book{ziegler2008srim,
  title={SRIM: the stopping and range of ions in matter},
  author={Ziegler, James F and Ziegler, Matthias D and Biersack, Jochen P},
  year={2008},
  publisher={Cadence Design Systems}
}
@article{federici2003key,
  title={Key ITER plasma edge and plasma--material interaction issues},
  author={Federici, G and Andrew, P and Barabaschi, P and Brooks, J and Doerner, R and Geier, A and Herrmann, A and Janeschitz, G and Krieger, K and Kukushkin, A and others},
  journal={Journal of Nuclear Materials},
  volume={313},
  pages={11--22},
  year={2003},
  publisher={Elsevier}
}
@article{brezinsek2015plasma,
  title={Plasma-surface interaction in the Be/W environment: conclusions drawn from the JET-ILW for ITER},
  author={Brezinsek, Sebastijan and JET-EFDA contributors and others},
  journal={Journal of nuclear materials},
  volume={463},
  pages={11--21},
  year={2015},
  publisher={Elsevier}
}
@article{federici2001plasma,
  title={Plasma-material interactions in current tokamaks and their implications for next step fusion reactors},
  author={Federici, Gianfranco and Skinner, Charles H and Brooks, Jeffrey N and Coad, Joseph Paul and Grisolia, Christian and Haasz, Anthony A and Hassanein, Ahmed and Philipps, Volker and Pitcher, C Spencer and Roth, Joachim and others},
  journal={Nuclear Fusion},
  volume={41},
  number={12},
  pages={1967},
  year={2001},
  publisher={IOP Publishing}
}
@article{brezinsek2013fuel,
  title={Fuel retention studies with the ITER-like wall in JET},
  author={Brezinsek, S and Loarer, T and Philipps, V and Esser, HG and Gr{\"u}nhagen, S and Smith, R and Felton, R and Banks, J and Belo, P and Boboc, A and others},
  journal={Nuclear Fusion},
  volume={53},
  number={8},
  pages={083023},
  year={2013},
  publisher={IOP Publishing}
}
@article{brezinsek2013residual,
  title={Residual carbon content in the initial ITER-Like Wall experiments at JET},
  author={Brezinsek, S and Jachmich, S and Stamp, MF and Meigs, AG and Coenen, JW and Krieger, K and Giroud, C and Groth, M and Philipps, V and Gr{\"u}nhagen, S and others},
  journal={Journal of Nuclear Materials},
  volume={438},
  pages={S303--S308},
  year={2013},
  publisher={Elsevier}
}
@article{okamoto1991phase,
  title={Phase diagrams of binary tungsten alloys},
  author={Okamoto, H and Tanner, LE and Naidu, SV Nagendra and Rao, P Ramo},
  journal={Indian Institute of Metals, Calcutta},
  year={1991}
}
@article{doerner2005beryllium,
  title={Beryllium--tungsten mixed-material interactions},
  author={Doerner, RP and Baldwin, MJ and Causey, RA},
  journal={Journal of nuclear materials},
  volume={342},
  number={1-3},
  pages={63--67},
  year={2005},
  publisher={Elsevier}
}
@article{baldwin2007w,
  title={Be--W alloy formation in static and divertor-plasma simulator experiments},
  author={Baldwin, MJ and Doerner, RP and Nishijima, D and Buchenauer, D and Clift, WM and Causey, RA and Schmid, K},
  journal={Journal of nuclear materials},
  volume={363},
  pages={1179--1183},
  year={2007},
  publisher={Elsevier}
}

@article{doerner2007implications,
  title={The implications of mixed-material plasma-facing surfaces in ITER},
  author={Doerner, RP},
  journal={Journal of nuclear materials},
  volume={363},
  pages={32--40},
  year={2007},
  publisher={Elsevier}
}
@article{linsmeier2007binary,
  title={Binary beryllium--tungsten mixed materials},
  author={Linsmeier, Ch and Ertl, K and Roth, J and Wiltner, A and Schmid, K and Kost, F and Bhattacharyya, SR and Baldwin, M and Doerner, RP},
  journal={Journal of nuclear materials},
  volume={363},
  pages={1129--1137},
  year={2007},
  publisher={Elsevier}
}
@article{bjorkas2010w,
  title={A Be--W interatomic potential},
  author={Bj{\"o}rkas, C and Henriksson, KOE and Probst, M and Nordlund, K},
  journal={Journal of Physics: Condensed Matter},
  volume={22},
  number={35},
  pages={352206},
  year={2010},
  publisher={IOP Publishing}
}
@article{lasa2014atomistic,
  title={Atomistic simulations of Be irradiation on W: mixed layer formation and erosion},
  author={Lasa, A and Heinola, K and Nordlund, K},
  journal={Nuclear Fusion},
  volume={54},
  number={8},
  pages={083001},
  year={2014},
  publisher={IOP Publishing}
}

@article{lasa2014effect,
  title={The effect of beryllium on deuterium implantation in tungsten by atomistic simulations},
  author={Lasa, A and Heinola, K and Nordlund, K},
  journal={Nuclear Fusion},
  volume={54},
  number={12},
  pages={123021},
  year={2014},
  publisher={IOP Publishing}
}
@article{thompson2015spectral,
  title={Spectral neighbor analysis method for automated generation of quantum-accurate interatomic potentials},
  author={Thompson, Aidan P and Swiler, Laura P and Trott, Christian R and Foiles, Stephen M and Tucker, Garritt J},
  journal={Journal of Computational Physics},
  volume={285},
  pages={316--330},
  year={2015},
  publisher={Elsevier}
}
@incollection{biersack1982stopping,
  title={The stopping and range of ions in solids},
  author={Biersack, JP and Ziegler, James F},
  booktitle={Ion implantation techniques},
  pages={122--156},
  year={1982},
  publisher={Springer, Berlin, Heidelberg}
}
@article{bartok2013representing,
  title={On representing chemical environments},
  author={Bart{\'o}k, Albert P and Kondor, Risi and Cs{\'a}nyi, G{\'a}bor},
  journal={Physical Review B},
  volume={87},
  number={18},
  pages={184115},
  year={2013},
  publisher={APS}
}
@article{bartok2010gaussian,
  title={Gaussian approximation potentials: The accuracy of quantum mechanics, without the electrons},
  author={Bart{\'o}k, Albert P and Payne, Mike C and Kondor, Risi and Cs{\'a}nyi, G{\'a}bor},
  journal={Physical review letters},
  volume={104},
  number={13},
  pages={136403},
  year={2010},
  publisher={APS}
}
@book{varshalovich1988quantum,
  title={Quantum theory of angular momentum},
  author={Varshalovich, Dmitri{\u\i} Aleksandrovich and Moskalev, Anatolij Nikolaevi{\v{c}} and Khersonskii, Valerii Kel'manovich},
  year={1988},
  publisher={World Scientific}
}
@article{plimpton1995fast,
  title={Fast parallel algorithms for short-range molecular dynamics},
  author={Plimpton, Steve},
  journal={Journal of computational physics},
  volume={117},
  number={1},
  pages={1--19},
  year={1995},
  publisher={Elsevier}
}
@inproceedings{trott2014snap,
  title={SNAP: strong scaling high fidelity molecular dynamics simulations on leadership-class computing platforms},
  author={Trott, Christian R and Hammond, Simon D and Thompson, Aidan P},
  booktitle={International Supercomputing Conference},
  pages={19--34},
  year={2014},
  organization={Springer}
}
@article{ziegler2010srim,
  title={SRIM--The stopping and range of ions in matter (2010)},
  author={Ziegler, James F and Ziegler, Matthias D and Biersack, Jochen P},
  journal={Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
  volume={268},
  number={11-12},
  pages={1818--1823},
  year={2010},
  publisher={North-Holland}
}
@article{marian2017recent,
  title={Recent advances in modeling and simulation of the exposure and response of tungsten to fusion energy conditions},
  author={Marian, Jaime and Becquart, Charlotte S and Domain, Christophe and Dudarev, Sergei L and Gilbert, Mark R and Kurtz, Richard J and Mason, Daniel R and Nordlund, Kai and Sand, Andrea E and Snead, Lance L and others},
  journal={Nuclear Fusion},
  volume={57},
  number={9},
  pages={092008},
  year={2017},
  publisher={IOP Publishing}
}
@article{kresse1993ab,
  title={Ab initio molecular dynamics for liquid metals},
  author={Kresse, Georg and Hafner, J{\"u}rgen},
  journal={Physical Review B},
  volume={47},
  number={1},
  pages={558},
  year={1993},
  publisher={APS}
}
@article{giannozzi2009quantum,
  title={QUANTUM ESPRESSO: a modular and open-source software project for quantum simulations of materials},
  author={Giannozzi, Paolo and Baroni, Stefano and Bonini, Nicola and Calandra, Matteo and Car, Roberto and Cavazzoni, Carlo and Ceresoli, Davide and Chiarotti, Guido L and Cococcioni, Matteo and Dabo, Ismaila and others},
  journal={Journal of physics: Condensed matter},
  volume={21},
  number={39},
  pages={395502},
  year={2009},
  publisher={IOP Publishing}
}
@article{soler2002siesta,
  title={The SIESTA method for ab initio order-N materials simulation},
  author={Soler, Jos{\'e} M and Artacho, Emilio and Gale, Julian D and Garc{\'\i}a, Alberto and Junquera, Javier and Ordej{\'o}n, Pablo and S{\'a}nchez-Portal, Daniel},
  journal={Journal of Physics: Condensed Matter},
  volume={14},
  number={11},
  pages={2745},
  year={2002},
  publisher={IOP Publishing}
}
@article{saal2013materials,
  title={Materials design and discovery with high-throughput density functional theory: the open quantum materials database (OQMD)},
  author={Saal, James E and Kirklin, Scott and Aykol, Muratahan and Meredig, Bryce and Wolverton, Christopher},
  journal={Jom},
  volume={65},
  number={11},
  pages={1501--1509},
  year={2013},
  publisher={Springer}
}
@article{jain2013commentary,
  title={Commentary: The Materials Project: A materials genome approach to accelerating materials innovation},
  author={Jain, Anubhav and Ong, Shyue Ping and Hautier, Geoffroy and Chen, Wei and Richards, William Davidson and Dacek, Stephen and Cholia, Shreyas and Gunter, Dan and Skinner, David and Ceder, Gerbrand and others},
  journal={Apl Materials},
  volume={1},
  number={1},
  pages={011002},
  year={2013},
  publisher={AIP}
}
@article{zhuang2013computational,
  title={Computational search for single-layer transition-metal dichalcogenide photocatalysts},
  author={Zhuang, Houlong L and Hennig, Richard G},
  journal={The Journal of Physical Chemistry C},
  volume={117},
  number={40},
  pages={20440--20445},
  year={2013},
  publisher={ACS Publications}
}
@article{villars2006asm,
  title={ASM alloy phase diagrams database},
  author={Villars, P and Okamoto, H and Cenzual, K},
  journal={ASM International, Materials Park, OH, USA},
  year={2006}
}
@article{daw1993embedded,
  title={The embedded-atom method: a review of theory and applications},
  author={Daw, Murray S and Foiles, Stephen M and Baskes, Michael I},
  journal={Materials Science Reports},
  volume={9},
  number={7-8},
  pages={251--310},
  year={1993},
  publisher={Elsevier}
}
@article{baskes1992modified,
  title={Modified embedded-atom potentials for cubic materials and impurities},
  author={Baskes, MI},
  journal={Physical review B},
  volume={46},
  number={5},
  pages={2727},
  year={1992},
  publisher={American Physical Society}
}
@article{sinnott2012three,
  title={Three decades of many-body potentials in materials research},
  author={Sinnott, Susan B and Brenner, Donald W},
  journal={Mrs Bulletin},
  volume={37},
  number={5},
  pages={469--473},
  year={2012},
  publisher={Cambridge University Press}
}
@article{liang2013reactive,
  title={Reactive potentials for advanced atomistic simulations},
  author={Liang, Tao and Shin, Yun Kyung and Cheng, Yu-Ting and Yilmaz, Dundar E and Vishnu, Karthik Guda and Verners, Osvalds and Zou, Chenyu and Phillpot, Simon R and Sinnott, Susan B and Van Duin, Adri CT},
  journal={Annual Review of Materials Research},
  volume={43},
  pages={109--129},
  year={2013},
  publisher={Annual Reviews}
}
@article{tersoff1988empirical,
  title={Empirical interatomic potential for silicon with improved elastic properties},
  author={Tersoff, Jerry},
  journal={Physical Review B},
  volume={38},
  number={14},
  pages={9902},
  year={1988},
  publisher={American Physical Society}
}
@article{lennard1931cohesion,
  title={Cohesion},
  author={Lennard-Jones, John E},
  journal={Proceedings of the Physical Society},
  volume={43},
  number={5},
  pages={461},
  year={1931},
  publisher={IOP Publishing}
}
@article{behler2007generalized,
  title={Generalized neural-network representation of high-dimensional potential-energy surfaces},
  author={Behler, J{\"o}rg and Parrinello, Michele},
  journal={Physical review letters},
  volume={98},
  number={14},
  pages={146401},
  year={2007},
  publisher={APS}
}
@article{behler2016perspective,
  title={Perspective: Machine learning potentials for atomistic simulations},
  author={Behler, J{\"o}rg},
  journal={The Journal of chemical physics},
  volume={145},
  number={17},
  pages={170901},
  year={2016},
  publisher={AIP Publishing}
}
@misc{rupp2018guest},
  title={Guest editorial: Special topic on data-enabled theoretical chemistry},
  author={Rupp, Matthias and von Lilienfeld, O Anatole and Burke, Kieron},
  year={2018},
  publisher={AIP Publishing}
}
@article{schutt2018schnet,
  title={SchNet--A deep learning architecture for molecules and materials},
  author={Sch{\"u}tt, Kristof T and Sauceda, Huziel E and Kindermans, P-J and Tkatchenko, Alexandre and M{\"u}ller, K-R},
  journal={The Journal of Chemical Physics},
  volume={148},
  number={24},
  pages={241722},
  year={2018},
  publisher={AIP Publishing}
}
@article{chen2017accurate,
  title={Accurate force field for molybdenum by machine learning large materials data},
  author={Chen, Chi and Deng, Zhi and Tran, Richard and Tang, Hanmei and Chu, Iek-Heng and Ong, Shyue Ping},
  journal={Physical Review Materials},
  volume={1},
  number={4},
  pages={043603},
  year={2017},
  publisher={APS}
}
@article{bartok2018machine,
  title={Machine learning a general purpose interatomic potential for silicon},
  author={Bartok, Albert P and Kermode, James and Bernstein, Noam and Csanyi, Gabor},
  journal={arXiv preprint arXiv:1805.01568},
  year={2018}
}
@article{wood2018extending,
  title={Extending the accuracy of the SNAP interatomic potential form},
  author={Wood, Mitchell A and Thompson, Aidan P},
  journal={The Journal of Chemical Physics},
  volume={148},
  number={24},
  pages={241721},
  year={2018},
  publisher={AIP Publishing}
}
@article{plimpton2012computational,
  title={Computational aspects of many-body potentials},
  author={Plimpton, Steven J and Thompson, Aidan P},
  journal={MRS bulletin},
  volume={37},
  number={5},
  pages={513--521},
  year={2012},
  publisher={Cambridge University Press}
}
@article{plimpton1995computational,
  title={Computational limits of classical molecular dynamics simulations},
  author={Plimpton, Steve},
  journal={Computational Materials Science},
  volume={4},
  number={4},
  pages={361--364},
  year={1995},
  publisher={Elsevier}
}
@article{ramprasad2017machine,
  title={Machine learning in materials informatics: recent applications and prospects},
  author={Ramprasad, Rampi and Batra, Rohit and Pilania, Ghanshyam and Mannodi-Kanakkithodi, Arun and Kim, Chiho},
  journal={npj Computational Materials},
  volume={3},
  number={1},
  pages={54},
  year={2017},
  publisher={Nature Publishing Group}
}
@article{botu2016machine,
  title={Machine learning force fields: construction, validation, and outlook},
  author={Botu, Venkatesh and Batra, Rohit and Chapman, James and Ramprasad, Rampi},
  journal={The Journal of Physical Chemistry C},
  volume={121},
  number={1},
  pages={511--522},
  year={2016},
  publisher={ACS Publications}
}
@article{lubbers2018hierarchical,
  title={Hierarchical modeling of molecular energies using a deep neural network},
  author={Lubbers, Nicholas and Smith, Justin S and Barros, Kipton},
  journal={The Journal of Chemical Physics},
  volume={148},
  number={24},
  pages={241715},
  year={2018},
  publisher={AIP Publishing}
}
@article{wang2018deepmd,
  title={DeePMD-kit: A deep learning package for many-body potential energy representation and molecular dynamics},
  author={Wang, Han and Zhang, Linfeng and Han, Jiequn and Weinan, E},
  journal={Computer Physics Communications},
  volume={228},
  pages={178--184},
  year={2018},
  publisher={Elsevier}
}
@article{kim2018polymer,
  title={Polymer Genome: A Data-Powered Polymer Informatics Platform for Property Predictions},
  author={Kim, Chiho and Chandrasekaran, Anand and Huan, Tran Doan and Das, Deya and Ramprasad, Rampi},
  journal={The Journal of Physical Chemistry C},
  volume={122},
  number={31},
  pages={17575--17585},
  year={2018},
  publisher={ACS Publications}
}
@article{botu2017study,
  title={A study of adatom ripening on an Al (111) surface with machine learning force fields},
  author={Botu, Venkatesh and Chapman, James and Ramprasad, Rampi},
  journal={Computational Materials Science},
  volume={129},
  pages={332--335},
  year={2017},
  publisher={Elsevier}
}
@article{mattox2018highly,
  title={Highly scalable discrete-particle simulations with novel coarse-graining: accessing the microscale},
  author={Mattox, Timothy I and Larentzos, James P and Moore, Stan G and Stone, Christopher P and Ibanez, Daniel A and Thompson, Aidan P and L{\'\i}sal, Martin and Brennan, John K and Plimpton, Steven J},
  journal={Molecular Physics},
  volume={116},
  number={15-16},
  pages={2061--2069},
  year={2018},
  publisher={Taylor \& Francis}
}
@article{csanyi2004learn,
  title={?Learn on the fly?: A hybrid classical and quantum-mechanical molecular dynamics simulation},
  author={Cs{\'a}nyi, Gabor and Albaret, T and Payne, MC and De Vita, A},
  journal={Physical review letters},
  volume={93},
  number={17},
  pages={175503},
  year={2004},
  publisher={American Physical Society}
}
@article{li2015molecular,
  title={Molecular dynamics with on-the-fly machine learning of quantum-mechanical forces},
  author={Li, Zhenwei and Kermode, James R and De Vita, Alessandro},
  journal={Physical review letters},
  volume={114},
  number={9},
  pages={096405},
  year={2015},
  publisher={APS}
}
@article{podryabinkin2017active,
  title={Active learning of linearly parametrized interatomic potentials},
  author={Podryabinkin, Evgeny V and Shapeev, Alexander V},
  journal={Computational Materials Science},
  volume={140},
  pages={171--180},
  year={2017},
  publisher={Elsevier}
}
@article{szlachta2014accuracy,
  title={Accuracy and transferability of Gaussian approximation potential models for tungsten},
  author={Szlachta, Wojciech J and Bart{\'o}k, Albert P and Cs{\'a}nyi, G{\'a}bor},
  journal={Physical Review B},
  volume={90},
  number={10},
  pages={104108},
  year={2014},
  publisher={APS}
}
@article{kresseInitioMolecularDynamics1993,
title={Ab initio molecular dynamics for liquid metals},
author={Kresse, Georg and Hafner, J{\"u}rgen},
journal={Physical Review B},
volume={47},
number={1},
pages={558},
year={1993},
publisher={APS}}

@article{kresseEfficientIterativeSchemes1996,
title={Efficient iterative schemes for ab initio
total-energy calculations using a plane-wave basis
set},
author={Kresse, Georg and Furthm{\"u}ller, J{\"u}rgen},
journal={Physical Review B},
volume={54},
number={16},
pages={11169},
year={1996},
publisher={APS}}

@article{kresseEfficiencyAbinitioTotal1996,
title={Efficiency of ab-initio total energy calculations
for metals and semiconductors using a plane-wave basis
set},
author={Kresse, Georg and Furthm{\"u}ller, J{\"u}rgen},
journal={Computational Materials Science},
volume={6},
number={1},
pages={15--50},
year={1996},
publisher={Elsevier}}

@article{perdewGeneralizedGradientApproximation1996,
title={Generalized gradient approximation made simple},
author={Perdew, John P and Burke, Kieron
and Ernzerhof, Matthias},
journal={Physical Review Letters},
volume={77},
number={18},
pages={3865},
year={1996},
publisher={APS}}

@article{blochl1994projector,
  title={Projector augmented-wave method},
  author={Bl{\"o}chl, Peter E},
  journal={Physical review B},
  volume={50},
  number={24},
  pages={17953},
  year={1994},
  publisher={APS}
}
@article{kresse1999ultrasoft,
  title={From ultrasoft pseudopotentials to the projector augmented-wave method},
  author={Kresse, Georg and Joubert, D},
  journal={Physical Review B},
  volume={59},
  number={3},
  pages={1758},
  year={1999},
  publisher={APS}
}
@misc{tikhonov2013numerical,
  title={Numerical methods for the solution of ill-posed problems},
  author={Tikhonov, Andre{\u\i} Nikolaevich and Goncharsky, A and Stepanov, VV and Yagola, Anatoly G},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@article{adams2009dakota,
  title={DAKOTA, a multilevel parallel object-oriented framework for design optimization, parameter estimation, uncertainty quantification, and sensitivity analysis: version 5.0 user?s manual},
  author={Adams, Brian M and Bohnhoff, WJ and Dalbey, KR and Eddy, JP and Eldred, MS and Gay, DM and Haskell, K and Hough, Patricia D and Swiler, Laura P},
  journal={Sandia National Laboratories, Tech. Rep. SAND2010-2183},
  year={2009}
}
@article{cusentino2015comparison,
  title={A comparison of interatomic potentials for modeling tungsten--hydrogen--helium plasma--surface interactions},
  author={Cusentino, Mary Alice and Hammond, Karl D and Sefta, Faiza and Juslin, Niklas and Wirth, Brian D},
  journal={Journal of Nuclear Materials},
  volume={463},
  pages={347--350},
  year={2015},
  publisher={Elsevier}
}
@article{juslin2013interatomic,
  title={Interatomic potentials for simulation of He bubble formation in W},
  author={Juslin, N and Wirth, BD},
  journal={Journal of Nuclear Materials},
  volume={432},
  number={1-3},
  pages={61--66},
  year={2013},
  publisher={Elsevier}
}
@article{derlet2007multiscale,
  title={Multiscale modeling of crowdion and vacancy defects in body-centered-cubic transition metals},
  author={Derlet, Peter M and Nguyen-Manh, D and Dudarev, SL},
  journal={Physical Review B},
  volume={76},
  number={5},
  pages={054107},
  year={2007},
  publisher={APS}
}
@article{lhuillier2011trapping,
  title={Trapping and release of helium in tungsten},
  author={Lhuillier, Pierre-Emile and Belhabib, Taieb and Desgardin, Pierre and Courtois, Blandine and Sauvage, Thierry and Barthe, Marie-France and Thomann, Anne-Lise and Brault, Pascal and Tessier, Yves},
  journal={Journal of Nuclear Materials},
  volume={416},
  number={1-2},
  pages={13--17},
  year={2011},
  publisher={Elsevier}
}
@article{silversmith1970pressure,
  title={Pressure dependence of the elastic constants of beryllium and beryllium-copper alloys},
  author={Silversmith, Donald J and Averbach, BL},
  journal={Physical Review B},
  volume={1},
  number={2},
  pages={567},
  year={1970},
  publisher={APS}
}
@misc{lammpsweb,
    title   = "{LAMMPS molecular dynamics package}",
    howpublished = "WWW site: \url{lammps.sandia.gov}",
    key = "LAMMPS",
}
@misc{libatoms,
    title   = "{libAtoms.org DFT data repository}",
    howpublished = "WWW site: \url{http://www.libatoms.org/Home/TungstenTrainingConfigurations}",
    key = "libAtoms.org",
}

% W-He
@article{parrinello1981polymorphic,
  title={Polymorphic transitions in single crystals: A new molecular dynamics method},
  author={Parrinello, Michele and Rahman, Aneesur},
  journal={Journal of Applied physics},
  volume={52},
  number={12},
  pages={7182--7190},
  year={1981},
  publisher={American Institute of Physics}
}
@article{tuckerman1992reversible,
  title={Reversible multiple time scale molecular dynamics},
  author={Tuckerman, MBBJM and Berne, Bruce J and Martyna, Glenn J},
  journal={The Journal of Chemical Physics},
  volume={97},
  number={3},
  pages={1990--2001},
  year={1992},
  publisher={American Institute of Physics}
}
@article{detemmerman2013,
  title={Helium effects on tungsten under fusion relevant plasma loading conditions},
  author={De Temmerman, G. and Bystrov, K. and Doerner, R.P. and Marot, L. and Wright, G.M. and Woller, K.B. and Whyte, D.G. and Zielinski, J.J.},
  journal={Journal of Nuclear Materials},
  volume={438},
  pages={S78-S83},
  year={2013},
}



@article{miyamoto2015,
  title={Systematic investigation of the formation behavior of helium bubbles in tungsten},
  author={Miyamoto, M. and Mikami, S. and Nagashima, H. and Iijima, N. and Nishijima, D. and Doerner, R.P. and Yoshida, N. and Watanabe, H. and Ueda, Y. and Sagara, A.},
  journal={Journal of Nuclear Materials},
  volume={463},
  pages={333-336},
  year={2015},
}


@article{klaver2016,
  title={Molecular dynamics simulations of ballistic He penetration into W fuzz},
  author={Klaver, T.P.C. and Nordlund, K. and Morgan, T.W. and Westerhof, E. and Thijsse, B.J. and van de Sanden, M.C.M},
  journal={Nuclear Fusion},
  volume={56},
  pages={126015},
  year={2016},
  publisher={IOP Publishing}
}
@article{pitts2013,
  title={A full tungsten divertor for ITER: Physics issues and design status},
  author={Pitts, R.A. and Carpenter, S. and Escourbiac, F. and Hirai, T. and Komarov, V. and Lisgo, S. and Kukushikin, A.S. and Loarte, A. and Merola, M. and Naik, A.S. and Mitteau, R. and Sugihara, M. and Bazylev, P. and Stangeby, P.C.},
  journal={Journal of Nuclear Materials},
  volume={438},
  pages={S48-S56},
  year={2013}
}
@article{federici2001,
  title={Plasma-material interactions in current tokamaks and their implications for the next step fusion reactors},
  author={Federici, G. and Skinner, C. and Brooks, J. and Coad, J. and Grisolia, C. and Hassz, A. and Hassanein, A. and Philipps, V. and Pitcher, C. and Roth, J. and Wampler, W. and Whyte, D.},
  journal={Nuclear Fusion},
  volume={41},
  pages={1967-2137},
  year={2001}
}
@article{wirth2015,
  title={Challenges and opportunities of modeling plasma-surface interactions in tungsten using high performance computing},
  author={Wirth, B.D. and Hammond, K.D. and Krasheninnikov, S.I. and Maroudas, D.},
  journal={Journal of Nuclear Materials},
  volume={463},
  pages={30-38},
  year={2015}
}
@article{baldwin2008,
  author={Baldwin, M.J. and Doerner, R.P.},
  title={Helium induced nanoscopic morphology on tungsten under fusion relevant plasma conditions},
  journal={Nuclear Fusion},
  volume={48},
  pages={038001},
  year={2008}
}
@article{baldwin2011,
  author={Baldwin, M.J. and Lynch, T.C., and Doerner, R.P. and Yu, J.H.},
  title={Nanostructure formation on tungsten exposed to low-pressure rf helium plasmas: A study of ion energy threshold and early stage growth},
  journal={Journal of Nuclear Materials},
  volume={415},
  pages={S104-S107},
  year={2011}
}
@article{hammond2014,
  author={Hammond, K.D. and Wirth, B.D.},
  title={Crystal orientation effects on helium ion depth distributions and adatom formation processes in plasma-facing tungsten},
  journal={Journal of Applied Physics},
  volume={116},
  pages={143301},
  year={2014}
}
@article{krasheninnikov2011,
  author={Krasheninnikov, S.I.},
  title={Viscoelastic model of tungsten 'fuzz' growth},
  journal={Physica Scripta},
  volume={T145},
  pages={014040},
  year={2011}
}
@article{kajita2009,
  author={Kajita, S. and Sakaguchi, W. and Ohno, N. and Yoshida, N. and Saeki, T.},
  title={Formation process of tunsten nanostructure by the exposure to helium plasma under fusion relevant plasma conditions},
  journal={Nuclear Fusion},
  volume={49},
  pages={095005},
  year={2009}
}
@article{kajita2007,
  author={Kajita, S. and Takamura, S. and Ohno, N. and Nishijima, D. and Iwakiri, H. and Yoshida, N.},
  title={Sub-ms laser pulse irradiation on tungsten target damaged by exposure to helium plasma},
  journal={Nuclear Fusion},
  volume={47},
  pages={1358-1366},
  year={2007}
}
@article{martynenko2012,
  author={Martynenko, Y.V and Nagel, M.Y.},
  title={Model of Fuzz Formation on a Tungsten Surface},
  journal={Plasma Physics Reports},
  volume={38},
  pages={996-999},
  year={2012}
}
@article{wright2013,
  author={Wright, G.M. and Brunner, D. and Baldwin, M.J. and Bystrov, K. and Doerner, R.P. and Labombard, B. and Lipschultz, B.and De Temmerman, G. and Terry, J.L. and Whyte, D.G. and Woller, K.B.},
  title={Comparison of tungsten nano-tendrils grwon in Alcator C-Mod and linear plasma devices},
  journal={Journal of Nuclear Materials},
  volume={438},
  pages={S84-S89},
  year={2013}
}
@article{borovikov2014,
  author={Borovikov, V. and Voter, A.F. and Tang, X.-Z.},
  title={Reflection and implantation of low energy hehlium with tungsten surfaces},
  journal={Journal of Nuclear Materials},
  volume={447},
  pages={254-270},
  year={2014}
}
@article{nishijima2004,
  author={Nishijima, D. and Ye, M.Y. and Ohno, N. and Takamura, S.},
  title={Formation mechanism of bubbles and holes on tungsten surface with low-energy and high-flux helium plasma irradiation in NAGDIS-II},
  journal={Journal of Nuclear Materials},
  volume={329-333},
  pages={1029-1033},
  year={2004}
}
@article{nishijima2003,
  author={Nishijima, D. and Ye, M.Y. and Ohno, N. and Takamura, S.},
  title={Incident ion energy dependence of bubble formation on tungsten surface with low energy and high flux helium plasma irradiation},
  journal={Journal of Nuclear Materials},
  volume={313-316},
  pages={97-101},
  year={2003}
}
@article{iwakiri2000,
  author={Iwakiri, H. and Yasunaga, K. and Morishita, K. and Yoshida, N.},
  title={Microstructure evolution in tungsten during low-energy helium ion irradiation},
  journal={Journal of Nuclear Materials},
  volume={283-287},
  pages={1134-1138},
  year={2000}
}
@article{takamura2006,
  author={Takamura, S. and Ohno, N. and Nishijima, D. and Kajita, S.},
  title={Formation of Nanostructured Tungsten with Arborescent Shape due to Helium Plasma Irradiation},
  journal={Plasma and Fusion Research},
  volume={1},
  pages={051},
  year={2006}
}
@article{baldwin2010,
  author={Baldwin, M.J. and Doerner, R.P.},
  title={Formation of helium induced nanostructure ‘fuzz’ on various tungsten grades},
  journal={Journal of Nuclear Materials},
  volume={404},
  pages={165-173},
  year={2010}
}
@article{kajita2011,
  author={Kajita, S. and Yoshida, N. and Yoshihara, R. and Ohno, N. and Yamagiwa, M.},
  title={TEM obervation of the growth process of helium nanonbubbles on tungsten: Nanostructure formation mechanism},
  journal={Journal of Nuclear Materials},
  volume={418},
  pages={152-158},
  year={2011}
}
@article{petty2015,
  author={Petty, T.J. and Baldwin, M.J. and Hasan, M.I. and Doerner, R.P. and Bradley, J.W.},
  title={Tungsten 'fuzz' growth re-examined: the dependence on ion fluence in non-erosive and erosive helium plasma},
  journal={Nuclear Fusion},
  volume={55},
  pages={09033},
  year={2015}
}
@article{hammond2017,
  author={Hammond, K.D.},
  title={Helium, hydrogen, and fuzz in plasma-facing materials},
  journal={Materials Research Express},
  volume={4},
  pages={104002},
  year={2017}
}
@article{nishijima2005,
  author={Nishijima, D. and Miyamoto, M. and Iwakiri, H. and Ye, M. and Ohno, N. and Tokunaga, K. and Yoshida, N. and Takamura, S.},
  title={Micron-Bubble Formation on Polycrystal Tungsten due to Low-Energy and High-Flux Helium Plasma Exposure},
  journal={Materials Transactions},
  volume={46},
  pages={561-564},
  year={2005}
}
@article{li2014,
  author={Li,X.-C. and Liu, Y.-N. and Luo, G.-N. and Shu, X. and Lu, G.-H.},
  title={Helium defects interactions and mechanism of helium bubble growth in tungsten: A molecular dynamics simulation},
  journal={Journal of Nuclear Materials},
  volume={451},
  pages={356-360},
  year={2014}
}
@article{ito2014,
  author={Ito, A.M. and Yoshimoto, Y. and Saito, S. and Takayama, A. and Nakamura, H.},
  title={Molecular dynamics simulation of a helium bubble bursting on tungsten surfaces },
  journal={Physica Scripta},
  volume={2014},
  pages={014062},
  year={2014}
}
@article{sefta2013,
  author={Sefta, F. and Hammond, K.D. and Juslin, N. and Wirth, B.D.},
  title={Tungsten surface evolution by helium bubble nucleation growth and rupture },
  journal={Nuclear Fusion},
  volume={2013},
  pages={073015},
  year={2013}
}
@techreport{hill1982,
     title = {Low Energy X-ray Emission from Magnetic Fusion Plasmas},
     author = {Hill, K.W. and Bitter, M. and Eames, D. and von Goeler, S. and Goldman, M. and Sauthoff, N.R. and Silver, E.},
     year = {1982},
     institution = {Princeton},
     month = {01},
     number= {PPPL-1807}
}
@article{umstadter2009,
  author={Umstadter, K.R. and Doerner, R. and Tynan, G.},
  title={Effect of bulk temperature on erosion of tungsten plasma-facing components subject to simultaneous deuterium plasma and heat pulses},
  journal={Physica Scripta},
  volume={2009},
  pages={014047},
  year={2009}
}
@article{plimpton1995,
  author={Plimpton, S.},
  title={Fast parallel algorithms for short-range molecular algorithms},
  journal={Journal of Computational Physics},
  volume={117},
  pages={1-19},
  year={1995}
}
@article{finnis1984,
  author={Finnis, M. and Sinclair, J.},
  title={A simple empirical n-body potential for transition metals},
  journal={Philisophical Magazine A},
  volume={50},
  pages={45-55},
  year={1984}
}
@article{ackland1987,
  author={Ackland, G.J. and Thetford R.},
  title={An improved n-body semi-empirical model for body-centered cubic transition metals},
  journal={Philisophical Magazine A},
  volume={56},
  pages={15-30},
  year={1987}
}
@article{juslin2013,
  author={Juslin, N. and Wirth, B.D.},
  title={Interatomic potentials for simulation of He bubble formation in W},
  journal={Journal of Nuclear Materials},
  volume={423},
  pages={61-66},
  year={2013}
}
@article{beck1968,
  author={Beck, D.},
  title={A new interatomic potential function for helium},
  journal={Molecular Physics},
  volume={14},
  pages={311-315},
  year={1968}
}
@article{morishita2003,
  author={Morishita, K. and Sugano, R. and Wirth, B.D. and de la Rubia, T.D.},
  title={Thermal Stability of helium-vacancy clusters in iron},
  journal={Nuclear Instruments and Methods in Physics Research Section B},
  volume={202},
  pages={76-81},
  year={2003}
}
@article{hammond2018,
  author={Hammond, K. and Blondel, S. and Hu, L. and Maroudas, D. and Wirth, D. },
  title={Large-scale atomistic simulations of low-energy helium implantation into tungsten single crystals},
  journal={Acta Materiala},
  volume={144},
  pages={561-578},
  year={2018}
}
@article{perez2014,
  author={Perez, D. and Vogel, T. and Uberuaga, B.P.},
  title={Diffusion and transformation kinetics of small helium clusters in bulk tungsten},
  journal={Physical Review B},
  volume={90},
  pages={014102},
  year={2014}
}
@BOOK{srim,
  TITLE = {The Stopping and Range of Ions in Solids},
  AUTHOR = {Ziegler, J.F. and Biersack, J.P. and Ziegler, M.D.},
  YEAR = {2008},
  PUBLISHER = {Springer},
  address={Morrisville},
  url={http://srim.org}
}
@article{dasgupta2019,
  author={Dasgupta, D. and Kolasinski, R.D. and Friddle, R.W. and Du, L. and Maroudas, D. and Wirth, B.D.},
  title={On the origin of fuzz formation in plasma facing materials},
  journal={Nuclear Fusion},
  volume={59},
  pages={086057},
  year={2019}
}
@article{wang2017,
  author={Wang, K. and Doerner, R.P. and Baldwin, M.J. and Meyer, F.W. and Bannister, M.E. and Darbal, A. and Stroud, R. and Parish, C.M.},
  title={Morphologies of tungsten nanotendrils grown under helium exposure},
  journal={Scientific Reports},
  volume={7},
  pages={42315},
  year={2017}
}
@article{stukowski2010,
  author={Stukowski, A.},
  title={Visualization and analysis of atomistic simulation data with OVITO - the Open Visualization Tool},
  journal={Modelling and Simulation in Material Science and Engineering},
  volume={18},
  pages={015012},
  year={2010}
}

@article{hu2015,
  author={Hu, L. and Hammond, K.D. and Wirth, B.D. and Maroudas, D.},
  title={Molecular-dynamics analysis of mobile helium cluster reactions near surfaces of plasma-exposed tungsten},
  journal={Journal of Applied Physics},
  volume={118},
  pages={163301},
  year={2015}
}

@article{becquart2007,
  author={Becquart, C.S. and Domain, C.},
  title={Ab initio calculations about intrinsic point defects and He in W},
  journal={Nuclear Instruments and Methods in Physics Research Section B: Beam Interactions with Materials and Atoms},
  volume={255},
  pages={23-26},
  year={2007}
}


%% W-Be References

@article{brezinsek2015,
  author={Brezinsek, S. and JET-EFDA contributors},
  title={Plasma-surface interaction in the Be/W environment: Conclusions drawn from the JET-ILW for ITER},
  journal={Journal of Nuclear Materials},
  volume={463},
  pages={11-21},
  year={2015}
}

@article{baldwin2007,
  author={Baldwin, M.J. and Doerner, R.P. and Nishijima, D. and Buchenauer, D. and Clift, W.M. and Causey, R.A. and Schmid, K.},
  title={Be-W alloy formation in static and divertor-plasma simulator experiments},
  journal={Journal of Nuclear Materials},
  volume={363-365},
  pages={1179-1183},
  year={2007}
}
@article{baldwin2009,
  author={Baldwin, M.J. and Doerner, R.P. and Nishijima, D. and Tokunaga, K. and Ueda, Y.},
  title={The effects of high fluence mixed-species (deuterium, helium, beryllium) plasma interactions with tungsten},
  journal={Journal of Nuclear Materials},
  volume={390-391},
  pages={886-890},
  year={2009}
}

@article{linsmeier2007,
  author={Linsmeier, Ch. and Ertl, K. and Roth, J. and Wiltner, A. and Schmid, K. and Kost, F. and Bhattacharyya, S.R. and Baldwin, M. and Doerner, R.P.},
  title={Binary beryllium-tungsten mixed materials},
  journal={Journal of Nuclear Materials},
  volume={363-365},
  pages={1129-1137},
  year={2007}
}

@article{lasa2015,
  author={Lasa, A. and Heinola, K. and Nordlund, K.},
  title={Atomistic simulations of Be irradiation on W: mixed layer formation and erosion},
  journal={Nuclear Fusion},
  volume={55},
  pages={099501},
  year={2015}
}

@article{lasa2014,
  author={Lasa, A. and Heinola, K. and Nordlund, K.},
  title={The effect of beryllium on deuterium implantation in tungsten by atomistic simulations},
  journal={Nuclear Fusion},
  volume={54},
  pages={123021},
  year={2014}
}


@book{okamoto1991,
  author={Okamoto, H. and Tanner, L.E.},
  title={Phase Diagrams of Binary Tungsten Alloys},
  publisher={Indian Institute of Metals},
  address={Calcutta},
  year={1991}
}

@article{detemmerman2008,
  author={De Temmerman, D. and Baldwin, M.J. and Doerner, R.P. and Nishijima, D. and Schmid, K.},
  title={An empirical scaling for deuterium retention in co-deposited beryllium layers},
  journal={Nuclear Fusion},
  volume={48},
  pages={075008},
  year={2008}
}

@article{bjorkas2010,
  author={Bjorkas, C. and K.O.E., Henriksson and Probst, M. and Nordlund, K.},
  title={A Be-W interatomic potential},
  journal={Journal of Physics: Condensed Matter},
  volume={22},
  pages={352206},
  year={2010}
}

% W-H

@article{condon1993,
  author={Condon, J.B. and Schober, T.},
  title={Hydrogen bubbles in metals},
  journal={Journal of Nuclear Materials},
  volume={207},
  pages={1-24},
  year={1993}
}

@article{causey2002,
  author={Causey, R.A.},
  title={Hydrogen isotope retention and recycling in fusion reactor plasma-facing components},
  journal={Journal of Nuclear Materials},
  volume={2002},
  pages={91-117},
  year={2002}
}

@article{haasz1999,
  author={Haasz, A. and Poon, M. and Davies, J.},
  title={The effect of ion damage on deuterium trapping in tungsten},
  journal={Journal of Nuclear Materials},
  volume={266-269},
  pages={520-525},
  year={1999}
}

@article{sze1999,
  author={Sze, F. and Doerner, R.P. and Luckhardt, S.},
  title={Investigation of plasma exposed W1\%La$_2$O$_3$ tungsten in a high ion flux, low energy, low carbon impurity plasma environment for the international thermonuclear experimental reactor},
  journal={Journal of Nuclear Materials},
  volume={264},
  pages={89-98},
  year={1999}
}
@article{venhaus2001,
  author={Venahus, T. and Causey, R. and Doerner, R.P. and Abeln, T.},
  title={Behavior of tungsten exposed to high fluences of low energy hydrogen isotopes},
  journal={Journal of Nuclear Materials},
  volume={290-293},
  pages={505-508},
  year={2001}
}
@article{ueda2009,
  author={Ueda, Y. and Fukumoto, M. and Yoshida, J. and Ohtsuka, Y. and Akiyoshi, R. and Iwakiri, H. and Yoshida, N.},
  title={Simultaneous irradiation effects of hydrogen and helium ions on tungsten},
  journal={Journal of Nuclear Materials},
  volume={386-388},
  pages={725-728},
  year={2009}
}

@article{miyamoto2009,
  author={Miyamoto, M. and Nishijima, D. and Ueda, Y. and Doerner, R.P. and Kurishita, H. and Baldwin, M.J. and Morito, S. and Ono, K. and Hanna, J.},
  title={Observations of suppressed retention and blistering for tungsten exposed to deuterium-helium mixture plasma},
  journal={Nuclear Fusion},
  volume={49},
  pages={065035},
  year={2009}
}

@article{ogorodnikova2011,
  author={Ogorodnikova, O.V. and Sugiyama, K. and Markin, A. and Gasparyan, Y. and Efimov, V. and Manhard, A. and Balden, M.},
  title={Effect of nitrogen seeding into deuterium plasma on deuterium retention in tungsten},
  journal={Physica Scripta},
  volume={T145},
  pages={014034},
  year={2011}
}
@article{oberkofler2016,
  author={Oberkofler, M. and Meisl, G. and Hakola, A. and Drenik, A. and Alegre, D. and Brezinsek, S. and Craven, R. and Dittmar, T. and Keenan, T. and Romanelli, S.G. and Smith, R. and Douai, D. and Herrmann, A. and Krieger, K. and Kruezi, U. and Liang, G. and Linsmeier, Ch. and Mozetic, M. and Rohde, V. and the ASDEX Upgrade team, the EUROfusion MST1 Team and JET Contributors},
  title={Nitrogen retention mechanisms in tokamaks with beryllium and tungsten plasma-facing surfaces},
  journal={Physica Scripta},
  volume={T167},
  pages={014077},
  year={2016}
}
@article{doerner2005,
  author={Doerner, R.P. and Baldwin, M.J. and Causey, R.A.},
  title={Beryllium-tungsten mixed-material interactions},
  journal={Journal of Nuclear Materials},
  volume={342},
  pages={63-67},
  year={2005}
}
@article{doerner2007,
  author={Doerner, R.P. and Baldwin, M.J. and Hanna, J. and Linsmeier, Ch. and Nishijima, D.},
  title={Interaction of beryllium containing plasma with ITER materials},
  journal={Physica Scripta},
  volume={T128},
  pages={115-120},
  year={2007}
}
@article{wood2019,
  author={Wood, M.A. and Cusentino, M.A. and Wirth, B.D. and Thompson, A.P.},
  title={Data-driven material models for atomistic simulation},
  journal={Physical Review B},
  volume={99},
  pages={184305},
  year={2019}
}

@article{thompson2015,
  author={Thompson, A.P. and Swiler, L.P. and Trott, C.R. and Foiles, S.M. and Tucker, G.J.},
  title={Spectral neighbor analysis method for automated generation of quantum-accurate interatomic potentials},
  journal={Journal of Computational Physics},
  volume={285},
  pages={316-330},
  year={2015}
}

@article{vladimirov2013,
  author={Vladimirov, P.V. and Moeslang, A.},
  title={Ab initio static and molecular dynamics sudies of helium behavior in beryllium},
  journal={Journal of Nuclear Materials},
  volume={442},
  pages={S694-S698},
  year={2013}
}

@techreport{dakota,
  author={Adamas, B.M. and Bohnhoff, W. and Dalbey, K. and Eddy, J. and Eldred, M. and Gay, D. and Haskell, K. and Hough, P.D. and Swiler, L.P.},
  title={DAKOTA: a multilevel parallel object-oriented framework for design optimization, parameter estimation, uncertainty quantification, and sensitivity analysis},
  number={SAND2010-2183},
  institution={Sandia National Laboratories},
  year={2009}
}

@article{boisse2014,
  author={Boisse, J. and De Backer, A. and Domain, C. and Becquart, C.S.},
  title={Modeling of the self trapping of helium and the trap mutation in tungsten using DFT and empirical potentials based on DFT},
  journal={Journal of Materials Research},
  volume={29},
  pages={2374-2386},
  year={2014}
}

@BOOK{was2017,
  TITLE = {Fundamentals of Radiation Materials Science},
  AUTHOR = {Was, G.},
  YEAR = {2017},
  PUBLISHER = {Springer},
  address={Morrisville},
}

@article{maroudas2016,
  author={Maroudas, D. and Blondel, S. and Hu, L. and Hammond, K.D. and Wirth, B.D.},
  title={Helium segregation on surfaces of plasma-exposed tungsten},
  journal={Journal of Physics: Condensed Matter},
  volume={28},
  pages={064004},
  year={2016}
}
